On Evaluating Performance of LLM Inference Serving Systems

The rapid evolution of Large Language Model (LLM) inference systems has yielded significant efficiency improvements. However, our systematic analysis reveals that current evaluation methodologies frequently exhibit fundamental flaws, often manifesting as common evaluation anti-patterns that obscure true performance characteristics and impede scientific progress. Through a comprehensive examination of recent systems, we identify recurring anti-patterns across three key dimensions: Baseline Fairness, Evaluation Setup, and Metric Design. These anti-patterns are uniquely problematic for LLM inference due to its dual-phase nature combining distinct prefill and decode operations, its handling of highly heterogeneous workloads, and its strict temporal requirements for interactive use. We demonstrate how common anti-patterns -- such as inadequate baseline comparisons that conflate engineering effort with algorithmic novelty, workload selections that fail to represent production scenarios, and metric normalizations that hide substantial performance variability like generation stalls-lead to misleading conclusions. To address these challenges, we provide a comprehensive checklist derived from our analysis, establishing a framework for recognizing and avoiding these anti-patterns in favor of robust LLM inference evaluation. To demonstrate the practical application of our framework, we present a case study analyzing speculative decoding, a technique whose bursty, non-uniform token generation is easily misinterpreted when evaluated using approaches characteristic of these anti-patterns. Our work establishes a rigorous foundation for evaluation methodology, enabling meaningful comparisons, ensuring reproducible results, and ultimately accelerating genuine progress in LLM inference systems by moving beyond common anti-patterns to align evaluation with real-world requirements.

==> 4-design.tex <==
\section{\sysname: Evaluation Framework}
\label{sec:design}

\input{fig-tex/fig-deadline-metric}

\subsection{Fluidity-Index: A User-Centric LLM Evaluation Metric}
\label{sec:design:fluidity-index}

To address the myriad of pitfalls associated with evaluation metrics, we propose a new evaluation metric which can holistically capture the user experience in online LLM inference serving systems. Inspired by video streaming quality metrics, we propose the \metric, which introduces token-level deadlines to measure generation consistency. Just as video playback requires frames to arrive before specific deadlines for smooth viewing, LLM applications need tokens to arrive at regular pace user consumption.

\input{fig-tex/fig-design-stall-time}
\input{algos/deadline_metric}

The key insight behind \metric is modeling token arrival expectations through a deadline-based approach. For a request starting at time t=0, we assign deadlines to both the prefill phase ($D_p$) and each subsequent decode token ($D_d$). As described in Algorithm~\autoref{alg:deadline}, a token arriving before its deadline, results in an accumulation of buffer time called \textit{slack} that can absorb future delays (line 13) in token generation for that request. This slack helps handle the natural variance in token generation times while maintaining a consistent user experience. When a token misses its deadline, the system resets subsequent deadlines while penalizing for all the missed deadlines due to stall (line 16). Thus, {\it \metric is the fraction of deadlines that were met for each of the output tokens for a given request and ranges between 0-1}.

This deadline-driven design captures both the magnitude and temporality of the token generation process. \autoref{fig:deadline:stall} demonstrates this through two scenarios, each experiencing a 4-second generation stall but at different points in the sequence. Both cases appear identical from the perspective of traditional metrics (P90 TBT: 40ms, TPOT: 46ms) but drastically different user-perceived performance. In the left graph, when the stall occurs early in generation, it caused a user-visible pause (fluidity=0.95). In contrast, the right graph shows the same stall occurring later in the sequence. By this point, the system has accumulated sufficient slack from previous early token arrivals, allowing it to absorb the stall without violating deadlines (fluidity=1.0).

The flexibility of \metric allows operators to define SLOs that precisely match their application requirements. A fluidity constraint of 1.0 corresponds to hard real-time systems where all token deadlines must be met. However, most LLM applications can tolerate some variation in token generation timing. For instance, an advanced voice interface (like OpenAI ChatGPT and Google Gemini) might require high fluidity (e.g., 0.9) to maintain natural speech flow, even if the absolute tokens-per-second requirement is lower than text interfaces. Conversely, applications focused primarily on completion time rather than generation smoothness, like code completion tools, might accept lower fluidity values. The percentile requirement (e.g., 99\% of requests meeting a fluidity threshold) ensures consistent performance across all users -- particularly important in production deployments where maintaining quality of service for tail users is crucial. This two-parameter SLO definition (percentile and fluidity threshold) provides operators fine-grained control over the tradeoff between generation smoothness and system capacity.

A critical aspect of performing robust evaluation using \metric is setting appropriate deadline targets. The prefill deadline $D_p$ must account for both the quadratic scaling of processing time with input length and scheduling delays in production deployments. To handle this, we split $D_p$ into two components: (1) a baseline prefill time determined by input length, and (2) a scheduling slack to absorb queueing delays. We use a reasonable open-source system like vLLM~\cite{vLLM:github} as baseline to benchmark the prefill time as a function of input length by profiling the request in isolation. We repeat this for 10 requests (tunable) and fit a curve through the observed points to obtain the baseline prefill target. The scheduling slack is then added to this baseline to create the final $D_p$ target, allowing operators to tune the slack based on their deployment requirements -- for instance, interactive applications might set a tight slack of 500ms while batch processing could allow several seconds. Note that, this is a recommendation on how to set the prefill latency target; different systems may observe different performance trends due to their implementation, optimizations, and kernels used. Therefore, the process of identifying this prefill latency curve should be repeated on the system being evaluated to set practical latency targets.









\subsection{Standardized Workload Suite}
\label{sec:design:workloads}

\sysname provides a set of standardized workloads drawn from open-source datasets that represent diverse LLM applications -- Conversation, Coding, Summarization, and Translation. These workloads exhibit varying prefill and decode characteristics, enabling comprehensive system evaluation across different deployment scenarios. It contains traces whose variations are frequently used in evaluations like \sharegpt, \lmsys and  \azurecode. The key statistics of these traces are captured in \autoref{table:workloads}.

For conversational workloads, we include \lmsys \cite{lmsyschat1m}, \sharegpt \cite{wang2023openchat}, and \mooncake \cite{mooncake}. Among these, \sharegpt offers the most balanced distribution with prefills up to 8K tokens and decodes up to 1K tokens, making it our recommended choice for evaluating chat applications. For development workflows, \azurecode \cite{azurepublicdataset} provides a large production trace (16.8M requests) with high prefill lengths (median 1.9K) but short decodes (median 8 tokens), ideal for testing compute-intensive prefill processing.

For long-context scenarios, we offer \arxivsum \cite{cohan-etal-2018-discourse} containing research paper-to-abstract pairs (median prefill 7.8K, decode 228) and \bwb \cite{jiang-etal-2022-blonde, jiang-etal-2023-discourse} translation trace (median prefill 2.4K, decode 3.6K). While \arxivsum tests compute capacity with large prefills, \bwb stresses memory systems with long decode sequences. For systems not targeting long contexts, we recommend filtering requests to prefill $<$ 16K and decode $<$ 1K tokens to maintain practical QPS rates during evaluation.







\subsection{Pluggable Evaluation Framework}
\label{sec:design:unified-deadline}

\sysname evaluation framework operates in two modes to support black-box API endpoints and self-managed  systems:

\vheading{Black-box Evaluation} \sysname evaluation framework operates in two modes to support both cloud API endpoints and self-hosted inference systems. The black-box evaluator interfaces with any OpenAI-compatible API endpoint, tracking token generation timestamps to measure both traditional metrics and \metric. In addition, \sysname also computes \rateMetric, which captures the stable token throughput that the system provide. This is achieved by identifying the minimum inter-token deadline ($D_d$) which satisfies user specified fluidity requirement, for example (e.g., 99\% of requests achieving 0.9 \metric).

\vheading{Capacity Evaluation} Our capacity evaluator employs an adaptive binary search to identify the maximum request load a system can sustain while meeting latency SLOs. The evaluator incrementally adjusts the load, monitoring both per-request metrics and system-wide fluidity distributions to determine stable operating points. 




\subsection{Implementation} We create a fork of open-source LLMPerf \cite{llmperf:github} which supports calling numerous LLM APIs, specifically, OpenAI compatible APIs~\cite{openaiapi}. We extend the codebase to support interacting with open-source LLM Inference Framework vLLM~\cite{vLLM:github}, calculating existing metrics discussed in ~\sref{sec:background:metrics}, \metric metric proposed in ~\sref{sec:design:unified-deadline} and capacity search.


==> algos/deadline_metric.tex <==
\begin{algorithm}[h]
\caption{\metric Computation}
\label{alg:deadline}
\begin{algorithmic}[1]
\REQUIRE \hspace{0.1em}\\        
     TBT Deadline: $D_d$, 
     Scheduling Slack: $S$, \\
     Prefill Tokens: $P$, 
     Inter Token Times: $T$\\
\ENSURE fluidity\_index
\STATE $D_p$ $\leftarrow$ predict\_prefill\_time($P$) + $S$
\STATE total\_deadlines $\leftarrow$ 0
\STATE missed\_deadlines $\leftarrow$ 0
\STATE slack $\leftarrow$ 0
\FOR{$i$ $\leftarrow$ 0 \textbf{to} length($T$) - 1}
\STATE $t$ $\leftarrow$ $T$[$i$]
\IF{$i$ == 0}
\STATE $D$ $\leftarrow$ $D_p$
\ELSE
\STATE $D$ $\leftarrow$ $D_d$
\ENDIF
\IF{$t$ $\leq$ $D$ + slack}
\STATE slack $\leftarrow$ slack + $D$ - $t$
\STATE total\_deadlines $\leftarrow$ total\_deadlines + 1
\ELSE
\STATE misses $\leftarrow$ ($t$ - slack - $D$) // $D_d$ + 1
\STATE missed\_deadlines $\leftarrow$ missed\_deadlines + misses
\STATE total\_deadlines $\leftarrow$ total\_deadlines + misses
\STATE slack $\leftarrow$ 0
\ENDIF
\ENDFOR \\
\textbf{return} 1 - missed\_deadlines / total\_deadlines
\end{algorithmic}
\end{algorithm}


==> fig-tex/fig-deadline-metric.tex <==
\begin{figure*}[t!]
\centering
\includegraphics[width=0.5\textwidth]{figs/deadline.pdf}
\caption{
    When a request arrives in the system, \sysname sets the deadlines for all future tokens. If a token is produced before the set deadline, the slack is carried forward and serves as a buffer for future tokens. When a token arrives late, the system gets penalized for all the missed deadlines, and the subsequent deadlines are reset to account for autoregressive decoding process.
    }
\label{fig:deadline:metric}
\end{figure*}
   



==> fig-tex/fig-design-stall-time.tex <==
\begin{figure}[htbp]
\centering
\includegraphics[width=0.5\linewidth]{figs/fluidity_temporal_corrected.pdf}
\caption{
    Demonstration of fluidity-index's temporal awareness in LLM token generation. Left: An early stall lead to missed deadlines (\metric=0.95). Right: The same stall occurring later is absorbed by accumulated slack (\metric=1.00). While both scenarios have identical P90 TBT (40ms) and TPOT (46ms), \metric captures how early stalls are more disruptive to user experience than later ones.
    }
\label{fig:deadline:stall}
\end{figure}
   



==> fig-tex/fig-mot-prefill.tex <==


\begin{figure}
\centering
\begin{subfigure}[b]{0.3\linewidth}
    \centering
    \includegraphics[width=\textwidth]{figs/yi-normalized-latency-cdf.pdf}
    \caption{\small Normalized Latency}
    \label{fig:mot:sd:norm_lat}
\end{subfigure}
\quad
\begin{subfigure}[b]{0.3\linewidth}
    \centering
    \includegraphics[width=\textwidth]{figs/yi-scheduling-delay-cdf.pdf}
    \caption{\small Scheduling Delay}
    \label{fig:mot:sd:sd}
\end{subfigure}
\caption{Normalized latency metric could be misleading due to scheduling delay obfuscation. On \arxivsum trace, 1.5 QPS, Yi-34B, while the scheduling delay is above 25s for  60\% requests in vLLM, the normalized latency only differs slightly.}
\label{fig:mot:sd}
\end{figure}


==> fig-tex/fig-open-source.tex <==



\begin{figure}[t!]
\centering
\begin{subfigure}[b]{0.21\textwidth}
    \centering
    \includegraphics[width=\textwidth, trim=12.2cm 0cm 0cm 1cm, clip]{figs/capacity_bars.pdf}
    \caption{\small System Capacity.}
    \label{fig:api:token-rate}
\end{subfigure}
\quad
\begin{subfigure}[b]{0.21\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figs/miss_rate_cdf.pdf}
    \caption{\small Deadline Miss Rate CDF.}
    \label{fig:api:tbt-latency}
\end{subfigure}
\caption{\small Capacity evaluation of open source systems vLLM and Sarathi-Serve performed on H100 for Llama3-8B. (a) shows the overall capacity achieved obtained by using different decode lat. metrics - TBT, TPOT, and \metric. (b) captures the distribution of deadline miss rate at capacity point for the two systems.}
\label{fig:eval:oss}
\end{figure}


==> fig-tex/fig-public-api.tex <==




\begin{figure}[t!]
\centering
\begin{subfigure}[b]{0.45\textwidth}
    \centering
    \includegraphics[width=\textwidth, trim=13cm 0cm 0cm 0cm, clip]{figs/token_rate_comparison_api.pdf}
    \caption{\small Token Generation Rate.}
    \label{fig:api:token-rate}
\end{subfigure}
\quad
\begin{subfigure}[b]{0.42\textwidth}
    \centering
    \includegraphics[width=\textwidth, trim=13cm 0cm 0cm 0cm, clip]{figs/tbt_cdf_api.pdf}
    \caption{\small TBT Latency Distribution.}
    \label{fig:api:tbt-latency}
\end{subfigure}
\quad
\begin{subfigure}[b]{0.45\textwidth}
    \centering
    \includegraphics[width=\textwidth, trim=13cm 0cm 0cm 0cm, clip]{figs/ttft_violin_plots.pdf}
    \caption{\small TTFT Distribution.}
    \label{fig:api:ttft}
\end{subfigure}
\quad
\begin{subfigure}[b]{0.42\textwidth}
    \centering
    \includegraphics[width=\textwidth, trim=13cm 0cm 0cm 0cm, clip]{figs/tbt_acceptance_rate_curve.pdf}
    \caption{\small Acceptance rate as a function of TBT target.}
    \label{fig:api:deadline}
\end{subfigure}
\caption{\small Evaluation of proprietary serving offerings for Mixtral-8x7B and Llama3-70B performed over duration of 24 hrs. (a) shows the token throughput as estimated by different decode latency metrics, (b) presents the overall decode latency distribution across all requests, (c) shows the TTFT for different prompt lengths and (d) provides a full characterization of the system by showing the \metric as a function of target TBT.}
\label{fig:api}
\end{figure}


==> math_commands.tex <==

\usepackage{amsmath,amsfonts,bm}

\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

\newcommand{\newterm}[1]{{\bf #1}}


\def\figref#1{figure~\ref{#1}}
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
\def\secref#1{section~\ref{#1}}
\def\Secref#1{Section~\ref{#1}}
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
\def\eqref#1{equation~\ref{#1}}
\def\Eqref#1{Equation~\ref{#1}}
\def\plaineqref#1{\ref{#1}}
\def\chapref#1{chapter~\ref{#1}}
\def\Chapref#1{Chapter~\ref{#1}}
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
\def\algref#1{algorithm~\ref{#1}}
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
\def\partref#1{part~\ref{#1}}
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdata}{p_{\rm{data}}}
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} %

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} %

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> outline.tex <==

\section{Introduction}
\paragraph{Opening}
\begin{itemize}
\item Rise of LLM inference systems and serving costs (thousands to millions per day)
\item Proliferation of serving solutions (open-source and proprietary)
\item Growing importance of accurate performance evaluation
\end{itemize}

\paragraph{Problem Statement}
\begin{itemize}
\item Current evaluation practices mask critical performance issues
\item Example: 3-4\myx claimed improvements hiding real usability problems
\item Systematic flaws in how the community evaluates systems
\end{itemize}

\paragraph{The Sins Framework}
\begin{itemize}
\item Overview of the three categories: system comparison, metric design, workload evaluation
\item Real-world impact of evaluation mistakes
\item Why traditional ML serving metrics fall short
\end{itemize}

\paragraph{Contributions}
\begin{itemize}
\item Systematic analysis of evaluation pitfalls with concrete examples
\item \sysname framework and fluidity-index metric
\item Comprehensive evaluation of existing systems
\item Open-source tools and methodology
\end{itemize}

\section{Background}
\subsection{LLM Inference Process}
\paragraph{Two-Phase Nature}
\begin{itemize}
\item Prefill phase: input processing, quadratic scaling
\item Decode phase: token-by-token generation
\item Memory requirements and scaling characteristics
\end{itemize}

\paragraph{KV Cache Dynamics}
\begin{itemize}
\item Purpose and benefits of KV caching
\item Memory-performance trade-offs
\item Impact on system capacity
\end{itemize}

\paragraph{System Constraints}
\begin{itemize}
\item GPU memory limitations
\item Batching considerations
\item CPU-GPU coordination overhead
\end{itemize}

\subsection{Traditional Evaluation Metrics}
\paragraph{Latency Metrics}
\begin{itemize}
\item TTFT: definition, use cases, limitations
\item TTLT: definition, use cases, limitations
\item TBT: measurement, importance for interactive applications
\item TPOT: calculation, common usage patterns
\item Normalized latency: calculation and typical usage
\end{itemize}

\paragraph{Throughput Metrics}
\begin{itemize}
\item System capacity measurements
\item QPS and token throughput metrics
\end{itemize}

\subsection{Challenges in LLM inference performance evaluations}
\paragraph{Unique characteristics of LLM inference}
\begin{itemize}
\item Each request has a unique compute requirement -- different number of prefill/decode tokens
\item Different latencies for each of prefill and decode phases
\item quadratic time complexity for prefill -- creating a gap between user expectations and what is computationally feasible 
\end{itemize}

\paragraph{Heterogeneous application requirements}
\begin{itemize}
\item Different metrics matter -- ttft, tbt, ttlt based on applications
\item varying latency requirements -- code - super strict, chat - somewhat relaxed, summaries - super relaxed
\item varying sensitivities to jitter -- advanced voice mode - low token tput is okay, but no jitters, copilot - only ttlt matters
\item varying seq lengths
\end{itemize}

\paragraph{Fast changing domain}


\section{The 12 Deadly Sins}

\subsection{System Comparison Sins}
\paragraph{Implementation Comparison Sin}
\begin{itemize}
\item Case study: nanoflow 1.9\myx improvement claim, but actual improvement 16\%
\item Impact of different engines and implementations
\item Need for microbenchmarking baselines
\end{itemize}

\paragraph{Baseline Tuning Sin}
\begin{itemize}
\item vLLM's fixed batch size of 8
\item chunk prefill misconfig in distserve and loongserve
\item Missing configuration optimizations
\item Impact on comparative results
\end{itemize}

\paragraph{Model Selection Sin}
\begin{itemize}
\item MHA vs GQA evaluation discrepancies
\item Impact on memory and performance characteristics
\item Case study: InfiniGen, other 
\end{itemize}

\subsection{Metric Design Sins}


\paragraph{Latency Normalization Issues}
\begin{itemize}
\item 25-second scheduling delays hidden by normalization
\item Case study: vLLM vs Sarathi-Serve comparison
\item Impact on user experience
\end{itemize}

\paragraph{Stall Masking}
\begin{itemize}
\item 10-second generation stalls in production
\item TPOT's failure to capture stall impact
\item Temporal aspects of performance
\end{itemize}

\paragraph{TTFT Problems}
\begin{itemize}
\item Quadratic scaling with input length
\item Static SLO impossibility
\item Real data on TTFT variation (512 to 32k tokens)
\end{itemize}

\paragraph{The wild west of evaluation metrics}
\begin{itemize}
\item Dozen different papers evaluating on different metics 
\item Several metrics are completely detached from actucal user facing metrics
\item Case study: input latency in loongserve, average latency in dLoRa
\end{itemize}

\subsection{Workload Sins}

\paragraph{Dataset Limitations}
\begin{itemize}
\item Single workload evaluations (e.g., ShareGPT only)
\item Fixed prompt length problems
\item Missing real-world workload characteristics
\item Very small requests length
\end{itemize}

\paragraph{Evaluation in unreasonable latency domains}
\begin{itemize}
\item Convoluted metrics often hide the fact that the latencies are not reasonable
\item Case study: learning to rank
\end{itemize}

\paragraph{SLO Inconsistencies}
\begin{itemize}
\item Varying definitions across papers
\item Impact on system comparisons
\item Need for standardization
\end{itemize}

\section{\sysname: A Holistic Approach}
\paragraph{Design Philosophy}
\begin{itemize}
\item Video streaming analogy
\item Deadline-based evaluation
\item User experience focus
\end{itemize}

\paragraph{Fluidity Metrics}
\begin{itemize}
\item Fluidity-index definition and rationale
\item Deadline calculation methodology
\item Buffer and recovery mechanics
\end{itemize}

\paragraph{Implementation Details}
\begin{itemize}
\item Black-box evaluation methodology
\item Capacity testing approach
\item Practical target setting
\end{itemize}

\section{Evaluation}


\paragraph{Design Insights}
\begin{itemize}
\item Impact of prefill strategies
\item Speculative decoding trade-offs
\item Resource scaling characteristics
\end{itemize}


\section{Related Work}
\paragraph{LLM Systems Evolution}
\begin{itemize}
\item Memory management advances
\item Scheduling strategies
\item Phase-specific optimizations
\end{itemize}

\paragraph{Evaluation Methodologies}
\begin{itemize}
\item Traditional ML serving metrics
\item Real-time systems theory
\item Streaming quality metrics
\end{itemize}

\section{Conclusion}
\paragraph{Impact Summary}
\begin{itemize}
\item Systematic evaluation improvements
\item New insights for system design
\item Practical deployment guidance
\end{itemize}

\paragraph{Future Directions}
\begin{itemize}
\item Standardization opportunities
\item Open research questions
\item Community collaboration needs
\end{itemize}


